Enhancing Question Answering for Enterprise Knowledge Bases using Large Language Models

Efficient knowledge management plays a pivotal role in augmenting both the operational efficiency and the innovative capacity of businesses and organizations. By indexing knowledge through vectorization, a variety of knowledge retrieval methods have emerged, significantly enhancing the efficacy of knowledge management systems. Recently, the rapid advancements in generative natural language processing technologies paved the way for generating precise and coherent answers after retrieving relevant documents tailored to user queries. However, for enterprise knowledge bases, assembling extensive training data from scratch for knowledge retrieval and generation is a formidable challenge due to the privacy and security policies of private data, frequently entailing substantial costs. To address the challenge above, in this paper, we propose EKRG, a novel Retrieval-Generation framework based on large language models (LLMs), expertly designed to enable question-answering for Enterprise Knowledge bases with limited annotation costs. Specifically, for the retrieval process, we first introduce an instruction-tuning method using an LLM to generate sufficient document-question pairs for training a knowledge retriever. This method, through carefully designed instructions, efficiently generates diverse questions for enterprise knowledge bases, encompassing both fact-oriented and solution-oriented knowledge. Additionally, we develop a relevance-aware teacher-student learning strategy to further enhance the efficiency of the training process. For the generation process, we propose a novel chain of thought (CoT) based fine-tuning method to empower the LLM-based generator to adeptly respond to user questions using retrieved documents. Finally, extensive experiments on real-world datasets have demonstrated the effectiveness of our proposed framework.

==> case.tex <==


\begin{table*}[t!]
\small
\caption{Case Study on the generation results.}
\begin{tabularx}{\textwidth}{X}
\toprule
\textbf{Q}: How to use real-time image defogging technology to solve the blur problem of images collected in foggy days?\\
\hline

\textbf{D \#1}: Aiming at the problems of low contrast and high noise in nighttime forest images, this research is dedicated to ... Technical research: Conduct in-depth research on various nighttime image enhancement methods, including\textcolor{green}{image fusion methods, dehazing model methods} and machine learning methods... \\

\textbf{D \#2}: Many features in images obtained in foggy environments are blurred, and the function of machine vision systems based on image features will be affected...\textcolor{red}{Based on the dark channel prior defogging algorithm, the image is dehazed through Matlab software}, the system parameters are adjusted to find the optimal solution for dehazing...\\

\textbf{D \#2}: If the image equipment collects images in foggy days, the collected images will have problems such as low brightness and blurred image outlines... developed using Xilinx FPGA, the core processor is Artix-7;  Image processing module: At the algorithm level, the atmospheric light transmission physical model and the dark channel method are used to\textcolor{red}{perform real-time dehazing and restoration processing of hazy images.} At the hardware level, the shift register implements the filtering function... \\

\hline

\textbf{A \#1}: This document examines ways to improve the quality of nighttime forest images. It does not introduce the specific defogging methods, so it is not relevant to the problem. Answer: Irrelevant.\\

\textbf{A \#2}: This document introduces how to eliminate haze on image imaging. This document proposes some relevant methods to the question. Answer: The first step is to improve the dark channel prior defogging algorithm. In the second step, the image is dehazed through matlab software. The third step is to adjust the system parameters to find the optimal solution for defogging. \\

\textbf{A \#2}: This document mainly solves the problem of blurred outlines in images collected in foggy days, and proposes solutions in terms of algorithms and hardware. This article provides specific solutions. Answer: The first step is to develop systems using Xilinx with the core processor Artix-7. The second step is to design an algorithm and use the physical model of atmospheric light transmission and the dark channel method to perform real-time dehazing and restoration processing of hazy images. In the fourth step, in the hardware implementation, a shift register is used to implement the filtering function.\\
\bottomrule
\end{tabularx}
\label{tab:Totto_case}
\end{table*}
